QuanTemp: A real-world open-domain benchmark for fact-checking numerical claims

Automated fact checking has gained immense interest to tackle the growing misinformation in the digital era. Existing systems primarily focus on synthetic claims on Wikipedia, and noteworthy progress has also been made on real-world claims. In this work, we release QuanTemp, a diverse, multi-domain dataset focused exclusively on numerical claims, encompassing temporal, statistical and diverse aspects with fine-grained metadata and an evidence collection without leakage. This addresses the challenge of verifying real-world numerical claims, which are complex and often lack precise information, not addressed by existing works that mainly focus on synthetic claims. We evaluate and quantify the limitations of existing solutions for the task of verifying numerical claims. We also evaluate claim decomposition based methods, numerical understanding based models and our best baselines achieves a macro-F1 of 58.32. This demonstrates that QuanTemp serves as a challenging evaluation set for numerical claim verification.

==> 01_introduction-AA.tex <==
\section{Introduction}

Online misinformation, particularly during elections, poses a significant threat to democracy by inciting socio-political and economic turmoil~\cite{vosoughi2018spread}. Fact-checking websites like \texttt{Politifact.com, Snopes.com, FullFact.org}, and others play an indispensable role in curbing misinformation. 
However, the scalability of manual fact-checking is constrained by limited resources. 
Manual fact-checking however is limited due to its time-consuming nature, scalability to the rapid spread of content produced, coupled with the need for specialized resources.
This limitation has spurred remarkable advancements in neural models for automated fact-checking in recent years~\cite{guo2022survey}, driven by increasing open datasets~\cite{thorne-etal-2018-fever, popat2018declare, chen2020tabfact, multifc, schlichtkrull2023averitec}.

\input{intro-example}

Within the area of fact-checking, the verification of claims involving numerical quantities and temporal expressions or \emph{numerical fact checking} is both essential and challenging. 
Numerical fact-checking is essential for countering the `numeric-truth-effect'\cite{sagara2009consumer} -- a significant component of political and social discourse -- where the presence of numbers can lend a false sense of credibility to a statement. 
For instance, our analysis of the \textsc{ClaimBuster dataset}~\cite{hassan2017toward} reveals that a substantial $36\%$ of all check-worthy claims in U.S. presidential debates involve numerical quantities or temporal expressions. \todo{point to section in the paper}.

Most current datasets inadequately address the verification of numerical claims, as our overview in Table~\ref{tab:datasets_overview} illustrates. 
A notable example is the \textsc{Feverous} dataset, where only a small fraction (approximately $10\%$) of claims necessitate numerical reasoning, and these have proven especially challenging for annotators to verify~\cite{aly2021feverous}. Our experiments further reinforce this difficulty. 
We observed that models trained on a mix of numerical and non-numerical claims underperform compared to those specifically fine-tuned on numerical claims.


Numerical claims verification poses a unique challenge, where a fact-checking system must critically analyze and reason about the numerical data presented in both the claim and its evidence. For example, in verifying the claim shown in Figure \ref{intro:example} as 'False', the NLI model needs to identify that the evidence only mentions 8 million households with incomes up to \$86k facing tax increases, contradicting the claim of tax increases for all families earning \$86k.

\input{table-datasets-comparison}

The existing datasets can be categorized as synthetically generated from Wikipedia and knowledge bases or real-world claims collected from fact-checking websites~(Table \ref{tab:datasets_overview}). While, works like \textsc{ClaimDecomp}~\cite{claimdecomp}, \textsc{MultiFC}~\cite{multifc} and \textsc{AveriTec}~\cite{schlichtkrull2023averitec}, collect real-world claims, they do not particularly focus on numerical claims. The only previous work proposing a dataset for fact-checking statistical claims, by \cite{vlachos_simple_numerical_1,numerical_claims_3}, uses a rule-based system to create synthetic claims from 16 simple statistical characteristics in the Freebase knowledge base about geographical regions. There has not been a dedicated \textbf{large-scale}, \textbf{real-world}, and \textbf{open-domain} diverse dataset for verifying \textbf{numerical claims}.

In this work, we collect and release a dataset of $15,514$ real-world claims with \textbf{numeric quantities and temporal expressions} from various fact-checking domains, complete with detailed metadata and an evidence corpus sourced from the web. \textit{Numeric claims are defined as statements needing verification of any explicit or implicit quantitative or temporal content}. 

The evidence collection method is crucial in fact-checking datasets. While datasets like \textsc{MultiFC} and \textsc{DeClarE} use claims as queries in search engines like Google and Bing for evidence, methods like \textsc{ClaimDecomp} depend on fact-checkers' justifications. However, this could cause `gold' evidence leakage from fact-checking sites into the training data. To avoid this, we  omit results from fact-checking websites in our evidence corpus.

Moreover, using claims as queries in search engines may miss crucial but non-explicit evidence for claim verification. To overcome this, recent works have proposed generating decomposed questions to retrieve better evidence \cite{QABriefs,claimdecomp,rani2023factify5wqa,aly-vlachos-2022-natural,claim_decompose}. In our approach, we aggregate evidence using both original claims and questions from methods like \textsc{ClaimDecomp} and \textsc{ProgramFC}. This dual strategy yields a more diverse and unbiased evidence set of \textbf{443,320 snippets}, enhancing which could be used for evaluating both the retrieval and NLI steps of fact-checking systems.

Finally, we also propose a fact-checking pipeline as a baseline that integrates claim decomposition techniques for evidence retrieval, along with a range of Natural Language Inference (NLI) models, encompassing pre-trained, fine-tuned, and generative approaches, to evaluate their efficacy on our dataset. Additionally, we conduct an error analysis, classifying the numerical claims into distinct categories to better understand the challenges they present.


\subsection{Research Questions}
In addition to collecting and releasing the dataset, we answer the following research questions by proposing a simple baseline system for fact-checking.

\mpara{RQ1}: How hard is the task of fact-checking numerical claims?

\mpara{RQ2}: To what extent does claim decomposition improve the verification of numerical claims?

\mpara{RQ3}: How effectively do models pre-trained for numeric understanding perform when fine-tuned to fact-check numerical claims?

\mpara{RQ4}: How does the size of large language models impact their performance in zero-shot, few-shot, and fine-tuned scenarios for numerical claims?

\subsection{Contributions}
\begin{itemize}[leftmargin=2pt,itemsep=0pt, topsep=0pt]
    \item We collect and release a large, diverse multi-domain dataset of real-world \textbf{15,514 numerical claims}, the first of its kind.

    \item We evaluate established fact-checking pipelines and claim decomposition methods, examining their \textbf{effectiveness in handling numerical claims}. Additionally, we propose improved baselines for the natural language inference (NLI) step.

    \item Our findings reveal that NLI models pre-trained for \textbf{numerical understanding outperform generic models} in fact-checking numerical claims by up to $11.78\%$. We also show that smaller models fine-tuned on numerical claims outperform larger models like GPT-3.5-Turbo under zero-shot and few-shot scenarios.

    \item We also \textbf{assess the quality of questions} decomposed by \textsc{ClaimDecomp} and \textsc{ProgramFC} for numerical claims, using both automated metrics and manual evaluation.
\end{itemize}

We make our dataset and code anonymously available here \url{https://anonymous.4open.science/r/QuanTemp-6DE5}.
x   

==> 09_limitations.tex <==
\section{Limitations}
\mpara{Evaluation of evidence retrieval:} Even though we collect an evidence corpus of $423,320$ snippets for the claims through Google search engine, we fix the retrieval stage to use BM25 first-stage retrieval and BERT-based re-ranking. However, it is not necessary that this is the most optimal setup for the fact-checking. There is a need for more thorough evaluation of the evidence retrieval step in the context of downstream fact-checking. In addition, use of better snippet selection methods could also improve the results.

\mpara{Temporal leakage:} While we extensively filter all results from fact-checking websites, we do not consider the temporal leakage avoidance proposed by \cite{schlichtkrull2023averitec}. There might be still be some web search results which are from non fact-checking domains and contain ready answer to the claim which are published after the claim was published. We estimate this is a minority of the cases. Moreover, as admitted by \cite{schlichtkrull2023averitec}, their temporal leakage avoidance is also not perfect since, claims are collected from multiple fact-checkers, some may have published the evidence earlier. In addition, from our experience, not all web pages have correct publication dates, which makes the exact dating of the evidence documents challenging.  

\mpara{Numerical Reasoning:} Since we deal with numerical claims, which tend to be complex in nature, there is a need for more complex numerical reasoning for the NLI step. In this work, we fine-tune and use models like \numt{}~\cite{yang2021nt5} and \finqaroberta{}~\cite{zhang2022elastic}, which are pre-trained on numerical understanding data and related tasks. However, these models do not directly perform numerical reasoning. Using the outcome of the numerical reasoning from the evidence provided by answer snippets of multiple questions for predicting the veracity could be a more effective way of fact-checking numerical claims. This approach deserves further research.

\section{Ethical Considerations and Risks}
\textbf{Credibility and bias of evidence sources:} Fact-checking is a sensitive process, while automated fact-checking systems assist in making some steps of the fact-checking process efficient, they are far from being fully automated. One critical challenge is the credibility of sources of evidence snippets. In this work, we use Google search engine to retrieve evidence which might introduce bias and trustworthiness issues. We predict the veracity of a claim purely based on the textual content of the evidence, but omit the credibility and trustworthiness of the source. Therefore, careful consideration is required before using this work as part of real-world fact-checking processes.

\textbf{Limitations of LLMs}: We employ LLMs for claim decomposition part of the pipeline and as a baseline for the NLI step, which has the risk of hallucination leading to incorrect information. While we control for hallucinations through by grounding the generation on demonstration samples, the effect might still persist. 

Additionally, we do not use any private information for the
proposed approach. Though some LLMs may have been pre-trained on
sensitive information, our prompts do not elicit any sensitive information directly or indirectly.


==> tab-results-final.tex <==
\begin{table*}[hbt!]
    \centering
    
    \begin{tabular}{lccccccccccccc}
    \toprule
     \textbf{Method}&\multicolumn{2}{c}{Statistical} & \multicolumn{2}{c}{Temporal} & \multicolumn{2}{c}{Interval} & \multicolumn{2}{c}{Comparison}& \multicolumn{2}{c}{Per-class F1} &\multicolumn{2}{c}{\numclaims{} Full} \\
   &\multicolumn{1}{c|}{M-F1} & \multicolumn{1}{c}{W-F1}&\multicolumn{1}{c|}{M-F1} & \multicolumn{1}{c}{W-F1}&\multicolumn{1}{c|}{M-F1} & \multicolumn{1}{c}{W-F1}&\multicolumn{1}{c|}{M-F1} & \multicolumn{1}{c}{W-F1} & \multicolumn{1}{c|}{T-F1} & \multicolumn{1}{c}{F-F1} & \multicolumn{1}{c|}{M-F1} & \multicolumn{1}{c}{W-F1} \\
     % & cover-EM & cover-EM& EM& EM&EM \\
     \midrule

     

    \midrule
    
    \textbf{Unified Evidence Corpus} & & \\
            Original Claim & 54.01 & 60.15 & 51.57& 68.69& 55.30 & 66.37 & 56.13 & 57.13& 36.10& 71.93 & 54.01 & 62.97 \\
          \programfc{} & 50.55 & 52.59  &  38.73& 47.73 & 47.86 & 54.78& \textbf{58.00} & \textbf{57.86}& 40.20 & 54.86  & 47.52 & 51.19\\

        \claimdecomp{} & 53.93 & 61.47 & 55.97 & 75.01& 58.67 & 72.84 & 54.21& 55.23 & 34.52& 77.04 & 55.78 & 66.41 \\

     \numdecomp{} & 53.00  & \textbf{63.65} &55.82& \textbf{79.70} & 54.37& \textbf{73.84}&46.12 & 47.87 &24.86 &83.00  & 53.93& \textbf{68.47} &  \\

     \midrule
     
          \textbf{Open Web} & & \\
        Original Claim & 46.19 & 46.33& 32.63& 41.39&40.36 & 46.29&61.15 &  60.97 & 38.54&47.43 & 42.98 & 45.20\\

     \programfc{} & 52.53& 54.85& 41.77 & 52.17 &  45.62& 52.23 & 56.12 & 56.10& \textbf{40.65} & 57.23 & 48.94 & 53.09\\
    \claimdecomp{} & 50.73 & 59.76 & 51.12 & 70.59 &48.78 & 66.22 & 48.84 & 50.15 & 26.53 & 74.94 & 50.73 & 62.84 \\

     \numdecomp{}&49.47 & 61.77 &52.62 & \textbf{77.83} & 53.16 & \textbf{73.25}  & 47.74&49.75 &19.15  & 83.04 & 51.09 & \textbf{67.07}  \\
     \midrule
\textbf{Oracle} & & & & & & & & & & \\ \midrule
Majority class &41.16 & 57.60 & 46.15 & 79.12 & 44.53 & 71.51 & 35.14& 38.09 & 0.00  &85.72& 42.86 & 64.30 \\
%          \textbf{Semi-Oracle} & & & & & & & & & & \\
%         ClaimOnly & 33.03& 39.57& 36.31 & 58.15 & 33.81& 48.61& 25.70 & 23.99&28.55 & 63.79 & 7.95 & 33.42 &  43.70  \\


% \programfc{} & 38.57& 42.49 & 37.12  & 50.66& 35.22& 45.76& 33.43&32.50 & 32.95 & 55.11 & 25.44 & 37.83 & 43.79 \\
%     \claimdecomp{}&33.43 & 39.78 & 35.04&  55.49 & 33.93 & 48.53& 34.37& 33.50&29.48 & 63.11& 10.85 & 34.48& 44.19  \\
%      \numdecomp{}& 33.81& 39.46 &33.57 & 53.45& 34.18& 47.00& 35.23&34.23 &29.11 & 60.29 & 13.90 &34.43& 43.24\\
     \bottomrule
    \end{tabular}
    \caption{Results across different categories of claims and combined results for \numclaims{}.}
    % \vspace{-1cm}
    \label{tab:main_result}
\end{table*}

==> tab-stance-ablations.tex <==
\begin{table}[hbt!]
% \small
\begin{tabular}{lcc}
% \begin{tabular}{lp{4.5cm}l}
\hline
\textbf{Model}  & \textbf{Macro-F1} & \textbf{Weighted-F1}  \\ 
\hline

\midrule
\programfc{}  & 78.20 & \\

\claimdecomp{}  &  \textbf{89.16}& \\
\numdecomp{}  & 86.62 & \\
 
\bottomrule
\end{tabular}
\caption{NLI model ablations}
\label{tab:stance_ablations}
\end{table}



==> table-ablations.tex <==
\begin{table}[ht!]
    \centering
     \scalebox{0.95}
    {
    \begin{tabular}{lcccccc}
    \toprule
     \textbf{Method}& \multicolumn{3}{c}{Per-class F1} &\multicolumn{2}{c}{\numclaims{} Full} \\
 & \multicolumn{1}{c|}{T-F1} & \multicolumn{1}{c|}{F-F1} & \multicolumn{1}{c}{C-F1} & \multicolumn{1}{c|}{M-F1} & \multicolumn{1}{c}{W-F1} \\
     % & cover-EM & cover-EM& EM& EM&EM \\
     \midrule

     

    % \midrule
    
    \textbf{Unified Evidence Corpus} & & \\

     % \numdecomp{}+\claimdecomp{}  \\
   %\ \textbf{Fine-tuned models} \\
         \bart{} & 51.23& 79.56 & 39.37 & 56.71 &64.54  \\

       %  Financial-Roberta-Large-MNLI & 54.12 & 58.73 & 61.62 & 77.23 & 53.43 & 64.20 & 54.31 & 54.02 & 48.16 & 77.95 & 44.39 &  56.83 & 64.25 \\
         Roberta-large &  50.58 & 77.23 &35.50&54.43 & 62.16 \\
         T5-small &  19.65 & 77.22 & 38.02 &  44.96 & 56.89 \\
      % \ \ \textbf{Numerical understanding } \\
         \numt{}  & 36.56 & 78.45 & 35.76 & 50.26 & 60.26  \\
         \finqaroberta{} & 49.72 & 77.91& \textbf{47.33} & \textbf{58.32} & \textbf{65.23}  \\
            % \ \textbf{Generative models (prompting)} \\


        FlanT5 (zero-shot) & 36.35 & 52.56& 3.15 & 30.68 & 37.64\\

          FlanT5 (few-shot)  & 33.90 & 54.73& 20.92 & 36.52 & 42.67\\
    \gptt{} (zero-shot) & 37.81 & 32.57& 31.25 & 33.87 & 33.25\\        
 \gptt{} (few-shot) &  44.41 & 64.26 & 32.35& 47.00 & 50.98 \\
 
    %  \midrule
     
    %       \textbf{Open Web} & & \\
    %     Original Claim &  \\

    %  \programfc{} &  \\
    % \claimdecomp{} &  \\

    %  \numdecomp{}&  \\
     \midrule
\textbf{Gold Evidence} \\


\gptt{} (few-shot)  & 56.77 & 75.35 & 28.00  & 53.37 & 60.47\\ 
 % \midrule
% Naive(Majority class) &22.46 & 34.25 & 28.35 & 62.95 & 25.86 & 49.19 & 16.51& 16.32& 0.00&  72.64 & 0.00  &24.21 & 41.42 \\


%          \textbf{Semi-Oracle} & & & & & & & & & & \\
%         ClaimOnly & 33.03& 39.57& 36.31 & 58.15 & 33.81& 48.61& 25.70 & 23.99&28.55 & 63.79 & 7.95 & 33.42 &  43.70  \\


% \programfc{} & 38.57& 42.49 & 37.12  & 50.66& 35.22& 45.76& 33.43&32.50 & 32.95 & 55.11 & 25.44 & 37.83 & 43.79 \\
%     \claimdecomp{}&33.43 & 39.78 & 35.04&  55.49 & 33.93 & 48.53& 34.37& 33.50&29.48 & 63.11& 10.85 & 34.48& 44.19  \\
%      \numdecomp{}& 33.81& 39.46 &33.57 & 53.45& 34.18& 47.00& 35.23&34.23 &29.11 & 60.29 & 13.90 &34.43& 43.24\\
     \bottomrule
    \end{tabular}}
    \caption{\footnotesize Ablation results employing different NLI models for \claimdecomp{} on \numclaims{}.}
    % \vspace{-1cm}
    \label{tab:ablations}
\end{table}

==> zero_shot_prompt.tex <==
\begin{table*}[ht]
% \scriptsize
\small
\caption{ \gptt{} zero shot for claim verification}
\begin{tabular}{p{17cm}}
\toprule 
\textbf{Prompts for zero-shot fact verification with \gptt{}. } 
% \midrule
\\
\midrule

% I am a highly intelligent question answering bot. If you ask me a question that is  \\
%   rooted in truth, I will give you the answer. If you ask me a question that is  \\  
%  nonsense, trickery, or has no clear answer, I will respond with 'Unknown'.\\ \\ 

\textbf{System prompt}: You are an expert fact checker.
        For the given claim, questions and evidences
        fact check the claim.   
            In the end generate the justification first and then the Label: 
           as strictly one of the labels SUPPORTS, REFUTES or CONFLICTING\\

\textbf{User Prompt}:
 For the given claim, questions and evidence
        fact check the claim, generate justification and output the label in the end.
        Classify the claim by predicting the Label: 
        as strictly one of the following: 
        SUPPORTS, REFUTES or CONFLICTING. Test claim: [Claim], Justification, Verdict:
\bottomrule
\end{tabular}

 \label{prompt:zero_shot}
\end{table*}
